Interpolating Discrete Diffusion Models with Controllable Resampling

Discrete diffusion models form a powerful class of generative models across diverse domains, including text and graphs. However, existing approaches face fundamental limitations. Masked diffusion models suffer from irreversible errors due to early unmasking, while uniform diffusion models, despite enabling self-correction, often yield low-quality samples due to their strong reliance on intermediate latent states. We introduce IDDM, an Interpolating Discrete Diffusion Model, that improves diffusion by reducing dependence on intermediate latent states. Central to IDDM is a controllable resampling mechanism that partially resets probability mass to the marginal distribution, mitigating error accumulation and enabling more effective token corrections. IDDM specifies a generative process whose transitions interpolate between staying at the current state, resampling from a prior, and flipping toward the target state, while enforcing marginal consistency and fully decoupling training from inference. We benchmark our model against state-of-the-art discrete diffusion models across molecular graph generation as well as text generation tasks, demonstrating competitive performance.

==> includes/bayesian_update.tex <==
Given a prior distribution $p(\x \mid \z)=\cat(\softmax(z)$ and an observation $\y\sim\mathcal{N}(\alpha \mathbf{e}_\x, \frac{1}{\beta}\mathbf{I})$, the posterior $p(\x\mid\z,\y)$ follows:
\begin{align}
        p(\x=c \mid \z)            & = \softmax(\z)_c \propto \exp(\z_{c})                                                             \\
        p(\y \mid \x=c)    & = \mathcal{N}(
        \alpha\ec, \frac{1}{\beta} \mathbf{I})                                                                                           \\
        p(\x=c \mid \z, \y) & = \propto p(\y \mid \x=c) \cdot p(\x=c \mid \z)                                           \\
                                      & = \mathcal{N}(\alpha\ec, \frac{1}{\beta}\mathbf{I}) \cdot \softmax(\z)_c             \\
                                      & \propto \exp\left(-\beta\frac{||\y - \alpha\ec||^2}{2}\right) \cdot \exp(\z_{c})                \\
                                      & = \exp\left(-\beta\frac{||\y||^2 - 2\alpha \cdot \y^T\ec + ||\alpha\ec||^2}{2} + \z_{c}\right) \\
                                      & \propto \exp\left(\alpha\beta \cdot \y_{c} + \z_{c}\right)
    \end{align}

    Let us now normalize the results to obtain the posterior probabilities:
    \begin{align}
        p(\x=c \mid \z, \y) & = \frac{\exp\left(\alpha\beta \cdot \y_{c} + \z_{c}\right)}{\sum_{c'\in\mathcal{C}} \exp\left(\alpha\beta \cdot \y_{c'} + \z_{c'}\right)} \\ &= \softmax(\z + \alpha\beta \cdot \y)_c
    \end{align}
    Putting everything together, we find that the posterior belief is $p(\x\mid \z,\y) =\cat(\x\mid \softmax(\z_\mathrm{post}))$ with
    \begin{equation}
        \z_\mathrm{post} = \z + \alpha\beta \cdot \y = \z + \frac{\alpha}{\beta}\epsilon
    \end{equation}

Therefore, $p(\z_\mathrm{post}\mid \z, \x)=\mathcal{N}(\alpha^2\beta\ex,\alpha\beta\mathbf{I}$).

% =========================
% Common setup (consistent notation)
% =========================
% Latent class is known (condition on x).
% Let C be the number of classes, and e_x \in R^C the one-hot vector for class x.
% Let z \in R^C be the (current) logit/state vector.

\newcommand{\Normal}{\mathcal{N}}
\newcommand{\e}{\mathbf{e}}

% ============================================================
% Option A: Direct (designed) Gaussian transition on logits
% Target: z_post | (z, x) ~ N(z + \gamma e_x, \beta I)
% ============================================================

\paragraph{Option A (direct Gaussian logit transition).}
Assume that the ground-truth class $x \in \{1,\dots,C\}$ is known and denote by $\e_x \in \mathbb{R}^C$ its one-hot encoding.
Fix two scalars $\alpha_t>0$ (information strength) and $\beta_t>0$ (noise variance).
Define the update
\begin{equation}
    \z_{t+1} \;=\; \z_t \;+\; \alpha_t\, \e_x \;+\; \sqrt{\beta_t}\,\varepsilon_t,
    \qquad \varepsilon_t \sim \Normal(0, I).
\end{equation}
Then, by affine-Gaussian transformation,
\begin{equation}
    \boxed{
    p(\z_{t+1} \mid \z_t, x)
    \;=\;
    \Normal\!\big(\z_t + \alpha_t\,\e_x,\; \beta_t I\big).
    }
\end{equation}
For our generative model we use:
\begin{equation}
    \boxed{
    p_\theta(\z_{t+1} \mid \z_t)
    \;=\;
    \Normal\!\big(\z_t + \alpha_tf_\theta(\z_t,t),\; \beta_t I\big).
    }
\end{equation}
\paragraph{ELBO}
Generative distribution $p_\theta(\x, \z_1, \dots,\z_k)=p(\x\mid \z_k)p_\theta(\z_k\mid \z_{k-1})\dots p_\theta(\z_1\mid \z_0)$ and encoding distribution $q(\z_1, \dots,\z_k\mid \x)=q(\z_k\mid \z_{k-1},\x)\dots q(\z_1\mid \z_0, \x)$
\begin{align}
    \log p(x) &\geq \mathbb{E}_{q(\z_1, \dots,\z_k\mid \x)}\left [ \log \frac{q(\z_1, \dots,\z_k\mid \x)}{p_\theta(\x, \z_1, \dots,\z_k)}\right ] \\
    &= \mathbb{E}_{q(\z_{i},\z_{i-1}\mid \x)}\left [ \log \frac{q(\z_i\mid \z_{i-1},\x)}{p_\theta(\z_i\mid\z_{i-1})}\right ] \\
    &= \mathbb{E}_{q(\z_{i-1}\mid \x)}\left [ \mathrm{KL}\left( q(\z_i\mid \z_{i-1},\x)\lVert p_\theta(\z_i\mid\z_{i-1}) \right )\right ] \\
    &= \mathbb{E}_{q(\z_{i-1}\mid\x)}\left[\frac{\alpha_{i-1}^2}{\beta_{t-1}}\lVert \e_x - \e_{\hat{x}} \rVert \right]
\end{align}
For $k\to\infty$:
\begin{align}
    \log p(x) = \mathbb{E}_{q(\z_{i-1}\mid\x)}\left[\frac{\alpha'_{i-1}^2}{\beta'_{t-1}}\lVert \e_x - \e_{\hat{x}} \rVert \right]
\end{align}

\clearpage
\paragraph{ELBO}
Generative distribution
\begin{equation}
    p_\theta(x, \z_1, \dots,\z_k)
    \;=\;
    p(x\mid \z_k)\prod_{i=0}^{k-1} p_\theta(\z_{i+1}\mid \z_i)
\end{equation}
and encoding distribution
\begin{equation}
    q(\z_1, \dots,\z_k\mid x)
    \;=\;
    \prod_{i=0}^{k-1} q(\z_{i+1}\mid \z_i,x).
\end{equation}
Then,
\begin{align}
    \log p_\theta(x)
    &\geq
    \mathbb{E}_{q(\z_1, \dots,\z_k\mid x)}\left[ \log \frac{p_\theta(x, \z_1, \dots,\z_k)}{q(\z_1, \dots,\z_k\mid x)}\right] \\
    &=
    \mathbb{E}_{q(\z_1, \dots,\z_k\mid x)}\!\left[\log p(x\mid \z_k)\right] \\
    \;&-\;
    \sum_{i=0}^{k-1}
    \mathbb{E}_{q(\z_i\mid x)}\!\left[
    \mathrm{KL}\!\left( q(\z_{i+1}\mid \z_i,x)\,\big\lVert\, p_\theta(\z_{i+1}\mid\z_i) \right)\right]. \label{eq:elbo_chain_ip1}
\end{align}
Moreover, for a fixed $i$, since both $q(\z_{i+1}\mid \z_i,x)$ and $p_\theta(\z_{i+1}\mid \z_i)$ are Gaussians with covariance $\beta_{i} I$,
\begin{align}
    \mathrm{KL}\!\left( q(\z_{i+1}\mid \z_i,x)\,\big\lVert\, p_\theta(\z_{i+1}\mid\z_i) \right)
    &=
    \frac{1}{2\beta_{i}}
    \left\|
    \big(\z_{i}+\alpha_{i}\e_x\big)
    -
    \big(\z_{i}+\alpha_{i} f_\theta(\z_{i},i)\big)
    \right\|_2^2 \\
    &=
    \frac{\alpha_{i}^2}{2\beta_{i}}
    \left\|
    \e_x - f_\theta(\z_{i},i)
    \right\|_2^2.
\end{align}
If one specializes to the case $f_\theta(\z_i,i)=\e_{\hat x}$ (i.e., a one-hot prediction),
\begin{align}
    \mathrm{KL}\!\left( q(\z_{i+1}\mid \z_i,x)\,\big\lVert\, p_\theta(\z_{i+1}\mid\z_i) \right)
    &=
    \frac{\alpha_{i}^2}{2\beta_{i}}
    \left\|
    \e_x - \e_{\hat x}
    \right\|_2^2.
\end{align}

\paragraph{Infinite-step (continuous-time) ELBO.}
Let $\Delta = 1/k$ and $t_i=i\Delta$. Assume the scaling
\[
\alpha_i=a(t_i)\Delta,\qquad \beta_i=b(t_i)\Delta,
\]
so that, as $k\to\infty$, the encoder process $q$ converges to
\[
d\z_t = a(t)\e_x\,dt + \sqrt{b(t)}\,dW_t,
\]
and the generative process $p_\theta$ converges to
\[
d\z_t = a(t)f_\theta(\z_t,t)\,dt + \sqrt{b(t)}\,dW_t.
\]
Then the ELBO becomes
\begin{align}
\log p_\theta(x)
\;\ge\;
\mathbb E_q\!\left[\log p(x\mid \z_1)\right]
\;-\;
\frac12\int_0^1
\mathbb E_q\!\left[
\frac{a(t)^2}{b(t)}\,
\big\|\e_x-f_\theta(\z_t,t)\big\|_2^2
\right]dt.
\label{eq:elbo_continuous}
\end{align}

\section{Discrete Update}
\begin{align}
    \pi_{t+1} = \begin{cases*}
        p_\theta(\pi_{t+1}\mid \pi_{t}) & if $m_{t+1}=0$ \\
        m_{t+1} & else
    \end{cases*}
\end{align}
% m_t in {0,1,...,C}; 0 = masked/soft, c>=1 = snapped to class c (absorbing)

\[
b_{t+1}\mid (m_t=0) \sim \Bernoulli(\gamma_{t+1}),
\qquad
\tilde x_{t+1}\mid (m_t=0,\pi_t) \sim \Cat(\pi_t),
\]
\[
m_{t+1} \;=\;
\begin{cases}
m_t, & m_t\in\{1,\dots,C\},\\
0,   & m_t=0 \ \text{and}\ b_{t+1}=0,\\
\tilde x_{t+1}, & m_t=0 \ \text{and}\ b_{t+1}=1.
\end{cases}
\]



% We introduce an auxiliary discrete state m_t that indicates whether we are still in the
% "soft" regime (probability simplex) or have already collapsed to a "hard" class.

% =========================
% Discrete diffusion "snapping" variable on top of simplex transitions
% =========================
\clearpage
% =========================
% Discrete diffusion "snapping" variable on top of simplex transitions
% =========================

\paragraph{Simplex state.}
Let $\z_t\in\mathbb{R}^C$ and $\pi_t \coloneqq \softmax(\z_t)\in\Delta^{C-1}$.

\paragraph{Discrete snapping state.}
Introduce a discrete variable
\[
m_t \in \{0,1,\dots,C\},
\]
where $m_t=0$ means \emph{not snapped yet} (we keep evolving $\pi_t$ on the simplex),
and $m_t=c\in\{1,\dots,C\}$ means \emph{snapped to class $c$} (an absorbing discrete state).

\paragraph{Forward noising (discrete diffusion) on $m_t$.}
Choose a schedule $\gamma_{t+1}\in[0,1]$ and define the forward (noising) Markov kernel
$q(m_{t+1}\mid m_t)$ by
\[
q(m_{t+1}=0 \mid m_t=0)=1,
\]
and for $c\in\{1,\dots,C\}$,
\[
q(m_{t+1}=c \mid m_t=c)=1-\gamma_{t+1},
\qquad
q(m_{t+1}=0 \mid m_t=c)=\gamma_{t+1},
\qquad
q(m_{t+1}=c' \mid m_t=c)=0\ \ (c'\neq c).
\]
Thus, a clean class is progressively \emph{masked} into state $0$; once masked, it stays masked.
This is an absorbing-state discrete diffusion (masking diffusion).

\paragraph{Reverse denoising (learned snapping) conditioned on the simplex state.}
We learn a reverse kernel $p_\phi(m_t\mid m_{t+1},\pi_{t+1})$ that (i) keeps absorbed classes fixed,
and (ii) when $m_{t+1}=0$ decides whether to remain masked or to snap to a class.
Parameterize it with two network heads:
\[
\hat\rho_{t+1} \;=\; \sigma\!\big(h_\phi(\pi_{t+1},t+1)\big)\in(0,1),
\qquad
\hat p_\phi(c\mid \pi_{t+1},t+1)\;=\;\softmax\!\big(g_\phi(\pi_{t+1},t+1)\big)_c.
\]
Then define
\[
p_\phi(m_t=c \mid m_{t+1}=c,\pi_{t+1}) = 1 \quad (c=1,\dots,C),
\]
and when $m_{t+1}=0$,
\[
p_\phi(m_t=0 \mid m_{t+1}=0,\pi_{t+1}) = 1-\hat\rho_{t+1},
\qquad
p_\phi(m_t=c \mid m_{t+1}=0,\pi_{t+1}) = \hat\rho_{t+1}\,\hat p_\phi(c\mid \pi_{t+1},t+1).
\]
Here $\hat\rho_{t+1}$ is the (learned) \emph{snapping probability} at step $t+1$; the categorical head
$\hat p_\phi(\cdot\mid \pi_{t+1},t+1)$ gives the snapped class distribution.

\paragraph{Coupling to the simplex transition.}
After sampling $m_{t+1}$, update the simplex state as
\[
\pi_{t+1}=
\begin{cases}
\text{sample from }p_\theta(\pi_{t+1}\mid \pi_t,t), & m_{t+1}=0,\\
\e_{m_{t+1}}, & m_{t+1}\in\{1,\dots,C\},
\end{cases}
\]
i.e., we keep denoising on the simplex while masked, and once snapped we set $\pi_{t+1}$ to the
corresponding corner (one-hot) and keep it there thereafter.


\clearpage
% ============================================================
% Hybrid model: simplex diffusion + discrete snapping diffusion
% ============================================================

\paragraph{State and notation.}
Let $\pi_t \in \Delta^{C-1}$ denote a simplex-valued state (e.g., $\pi_t=\softmax(\z_t)$ for logits $\z_t\in\mathbb{R}^C$).
Introduce a discrete \emph{snapping state}
\[
m_t \in \{0,1,\dots,C\},
\]
where $m_t=0$ means \emph{not snapped} (we keep evolving on the simplex), and $m_t=c\in\{1,\dots,C\}$ means \emph{snapped to class $c$}.
We write $\e_c\in\mathbb{R}^C$ for the one-hot corner.

\paragraph{Generative model.}
Fix a horizon $K$. Define a joint latent-variable model with latents $(m_{0:K},\pi_{0:K})$ and observation $x\in\{1,\dots,C\}$:
\begin{align}
p_{\theta,\phi}(x, m_{0:K}, \pi_{0:K})
&=
p(\pi_0)\,p(m_0)\,
\prod_{t=0}^{K-1} p_\phi(m_{t+1}\mid m_t,\pi_t)\;
\prod_{t=0}^{K-1} p_\theta(\pi_{t+1}\mid \pi_t, m_{t+1})\;
p(x\mid \pi_K).
\label{eq:joint_hybrid}
\end{align}
We choose the likelihood
\[
p(x\mid \pi_K)=\Cat(\pi_K).
\]
To encode the ``keep denoising if masked, otherwise keep the class/corner'', define
\[
p_\theta(\pi_{t+1}\mid \pi_t, m_{t+1}) \;=\;
\begin{cases}
p_\theta(\pi_{t+1}\mid \pi_t,t), & m_{t+1}=0,\\
\delta_{\e_{m_{t+1}}}(\pi_{t+1}), & m_{t+1}\in\{1,\dots,C\},
\end{cases}
\]
i.e., if a class is present we set $\pi_{t+1}$ deterministically to the corresponding corner.\footnote{In practice, to avoid measure-theoretic issues with Dirac deltas in KL terms, one typically enforces the same deterministic coupling in the variational distribution (see below), so the corresponding KL terms are identically zero.}

\paragraph{Variational (encoding) distribution.}
Let the variational posterior factorize as
\begin{align}
q(m_{0:K},\pi_{0:K}\mid x)
&=
q(m_0)\,q(\pi_0)\,
\prod_{t=0}^{K-1} q(m_{t+1}\mid m_t,x)\;
\prod_{t=0}^{K-1} q(\pi_{t+1}\mid \pi_t, x, m_{t+1}).
\label{eq:q_factor}
\end{align}
We mirror the same ``masked vs snapped'' structure:
\[
q(\pi_{t+1}\mid \pi_t, x, m_{t+1}) \;=\;
\begin{cases}
q(\pi_{t+1}\mid \pi_t,x,t), & m_{t+1}=0,\\
\delta_{\e_{m_{t+1}}}(\pi_{t+1}), & m_{t+1}\in\{1,\dots,C\}.
\end{cases}
\]
Here $q(m_{t+1}\mid m_t,x)$ is your \emph{forward discrete diffusion} (e.g. a masking noising kernel), and
$q(\pi_{t+1}\mid \pi_t,x,t)$ is your simplex/logit forward kernel (e.g. the Gaussian logit transition conditioned on the ground-truth class).

\paragraph{ELBO.}
By Jensen's inequality,
\begin{align}
\log p_{\theta,\phi}(x)
&\ge
\mathbb{E}_{q(m_{0:K},\pi_{0:K}\mid x)}
\left[
\log \frac{p_{\theta,\phi}(x,m_{0:K},\pi_{0:K})}{q(m_{0:K},\pi_{0:K}\mid x)}
\right]
\;\eqqcolon\; \mathcal{L}(\theta,\phi).
\end{align}
Expanding using~\eqref{eq:joint_hybrid} and~\eqref{eq:q_factor} yields the decomposition
\begin{align}
\mathcal{L}(\theta,\phi)
&=
\mathbb{E}_{q}\!\left[\log p(x\mid \pi_K)\right]
-\sum_{t=0}^{K-1}\mathbb{E}_{q}\!\left[
\mathrm{KL}\!\left(q(m_{t+1}\mid m_t,x)\,\big\|\,p_\phi(m_{t+1}\mid m_t,\pi_t)\right)\right]
\nonumber\\
&\quad
-\sum_{t=0}^{K-1}\mathbb{E}_{q}\!\left[
\mathrm{KL}\!\left(q(\pi_{t+1}\mid \pi_t,x,m_{t+1})\,\big\|\,p_\theta(\pi_{t+1}\mid \pi_t,m_{t+1})\right)\right]
\nonumber\\
&\quad
-\mathrm{KL}\!\left(q(m_0)\,\|\,p(m_0)\right)
-\mathrm{KL}\!\left(q(\pi_0)\,\|\,p(\pi_0)\right).
\label{eq:elbo_hybrid_full}
\end{align}

\paragraph{Gated continuous KL (masked steps only).}
Because both $q(\pi_{t+1}\mid \pi_t,x,m_{t+1})$ and $p_\theta(\pi_{t+1}\mid \pi_t,m_{t+1})$
use the \emph{same} deterministic corner mapping when $m_{t+1}\neq 0$, the continuous KL term vanishes there.
Hence the second sum reduces to
\begin{align}
\sum_{t=0}^{K-1}\mathbb{E}_{q}\!\left[
\mathrm{KL}\!\left(q(\pi_{t+1}\mid \pi_t,x,m_{t+1})\,\|\,p_\theta(\pi_{t+1}\mid \pi_t,m_{t+1})\right)\right]
=
\sum_{t=0}^{K-1}\mathbb{E}_{q}\!\left[
\mathbf{1}\{m_{t+1}=0\}\,
\mathrm{KL}\!\left(q(\pi_{t+1}\mid \pi_t,x,t)\,\|\,p_\theta(\pi_{t+1}\mid \pi_t,t)\right)\right].
\label{eq:gated_KL}
\end{align}

% Optional: if you instantiate q and p_theta as Gaussians in logits z,
% this KL becomes the familiar (alpha^2/(2 beta)) * ||e_x - f_theta||^2, multiplied by 1{m_{t+1}=0}.


% -------------------------------
% Discrete diffusion KL term (masking diffusion over m_t)
% -------------------------------
% State space: m_t \in {0,1,...,C}, where 0 = masked, c>=1 = class c.

% Forward (encoder) kernel q(m_{t+1} | m_t, x) for masking diffusion:
%   - if already masked: stay masked
%   - if in class c: mask with prob gamma_{t+1}, otherwise keep c
\[
q(m_{t+1}\mid m_t,x)=
\begin{cases}
\delta_0(m_{t+1}), & m_t=0,\\[2mm]
\gamma_{t+1}\,\delta_0(m_{t+1}) + (1-\gamma_{t+1})\,\delta_{m_t}(m_{t+1}), & m_t\in\{1,\dots,C\},
\end{cases}
\]
where $\delta_a(\cdot)$ denotes the Dirac mass at $a$ on the discrete space.

% Learned reverse (decoder) kernel p_\phi(m_t | m_{t+1}, \pi_{t+1}) (or p_\phi(m_{t+1}|m_t,\pi_t), depending on your direction):
% Here we write the KL term in the direction that appears in the ELBO:
\[
\mathcal{L}^{(m)}_{\mathrm{KL}}
\;\coloneqq\;
\sum_{t=0}^{K-1}
\mathbb{E}_{q(m_t,\pi_t\mid x)}
\Big[
\mathrm{KL}\big(q(m_{t+1}\mid m_t,x)\,\|\,p_\phi(m_{t+1}\mid m_t,\pi_t)\big)
\Big].
\]

% Closed form of the per-step KL under the masking forward kernel:
\[
\mathrm{KL}\big(q(m_{t+1}\mid m_t,x)\,\|\,p_\phi(m_{t+1}\mid m_t,\pi_t)\big)
=
\begin{cases}
-\log p_\phi(0\mid 0,\pi_t), & m_t=0,\\[1mm]
\gamma_{t+1}\log\frac{\gamma_{t+1}}{p_\phi(0\mid m_t,\pi_t)}
+(1-\gamma_{t+1})\log\frac{1-\gamma_{t+1}}{p_\phi(m_t\mid m_t,\pi_t)},
& m_t\in\{1,\dots,C\}.
\end{cases}
\]


==> includes/ctmc.tex <==
% CTMC version (finite state space): "refresh / restart" construction and proof via Kolmogorov forward equation.
% Requires: \usepackage{amsmath,amssymb}

\newcommand{\X}{\mathcal{X}}
\newcommand{\1}{\mathbf{1}}
\newcommand{\I}{\mathbf{I}}

\paragraph{Base CTMC (Markov) forward.}
Let $X(t)$ be a time-inhomogeneous CTMC on a finite state space $\X$ with generator (rate matrix) $R(t)$.
Write the (row) marginal distribution as
\[
\mu^{\mathrm{abs}}(t) \in \Delta^{|\X|-1},
\qquad
\mu^{\mathrm{abs}}_j(t) := \Pr(X(t)=j \mid X(0)=x_0).
\]
The Kolmogorov forward equation is
\begin{equation}
\frac{d}{dt}\mu^{\mathrm{abs}}(t) \;=\; \mu^{\mathrm{abs}}(t)\,R(t),
\qquad
\mu^{\mathrm{abs}}(0)=\delta_{x_0}.
\label{eq:KFE-base}
\end{equation}

\paragraph{Non-Markov ``refresh from $x_0$'' CTMC (conditionally Markov).}
Fix a nonnegative refresh rate $\lambda(t)\ge 0$.
Define a new CTMC (conditional on $x_0$) with generator
\begin{equation}
K(t)
\;:=\;
R(t) \;+\; \lambda(t)\big(\1\,\mu^{\mathrm{abs}}(t) - \I\big).
\label{eq:K-def}
\end{equation}
Equivalently, the additional (refresh) jump rates are, for $i\neq j$,
\begin{equation}
K_{ij}(t) \;=\; R_{ij}(t) \;+\; \lambda(t)\,\mu^{\mathrm{abs}}_j(t),
\qquad
K_{ii}(t) \;=\; -\sum_{j\neq i}K_{ij}(t),
\label{eq:K-entries}
\end{equation}
i.e. \emph{from any current state $i$, a refresh event occurs at rate $\lambda(t)$ and then the chain jumps to a new state $j$
distributed as $\mu^{\mathrm{abs}}(t)$ (which depends on $x_0$).}

Let $\mu^{\mathrm{nm}}(t)$ denote the marginal of this refreshed process:
\[
\mu^{\mathrm{nm}}_j(t) := \Pr(X_{\mathrm{nm}}(t)=j \mid X_{\mathrm{nm}}(0)=x_0),
\qquad
\mu^{\mathrm{nm}}(0)=\delta_{x_0}.
\]
Then $\mu^{\mathrm{nm}}$ satisfies the forward equation
\begin{equation}
\frac{d}{dt}\mu^{\mathrm{nm}}(t) \;=\; \mu^{\mathrm{nm}}(t)\,K(t).
\label{eq:KFE-nm}
\end{equation}

\paragraph{Claim (marginals are unchanged).}
For all $t\ge 0$,
\begin{equation}
\mu^{\mathrm{nm}}(t) \;=\; \mu^{\mathrm{abs}}(t),
\qquad\text{i.e.}\qquad
q_{\mathrm{nm}}(X(t)=\cdot \mid x_0) = q_{\mathrm{abs}}(X(t)=\cdot \mid x_0).
\label{eq:marginal-equality}
\end{equation}

\paragraph{Proof (Kolmogorov forward equation).}
We show that $\mu^{\mathrm{abs}}(t)$ also solves \eqref{eq:KFE-nm}.
Using \eqref{eq:K-def},
\begin{align}
\mu^{\mathrm{abs}}(t)\,K(t)
&=\mu^{\mathrm{abs}}(t)\,R(t)
\;+\;\lambda(t)\,\mu^{\mathrm{abs}}(t)\big(\1\,\mu^{\mathrm{abs}}(t) - \I\big)\\
&=\mu^{\mathrm{abs}}(t)\,R(t)
\;+\;\lambda(t)\Big( \underbrace{\mu^{\mathrm{abs}}(t)\1}_{=\,1}\,\mu^{\mathrm{abs}}(t) - \mu^{\mathrm{abs}}(t)\Big)\\
&=\mu^{\mathrm{abs}}(t)\,R(t).
\end{align}
Hence, by \eqref{eq:KFE-base},
\[
\frac{d}{dt}\mu^{\mathrm{abs}}(t) \;=\; \mu^{\mathrm{abs}}(t)\,R(t) \;=\; \mu^{\mathrm{abs}}(t)\,K(t).
\]
So $\mu^{\mathrm{abs}}$ and $\mu^{\mathrm{nm}}$ solve the same linear ODE \eqref{eq:KFE-nm} with the same initial condition,
and therefore coincide for all $t$ (uniqueness of solutions of linear ODEs). This proves \eqref{eq:marginal-equality}.

\paragraph{Infinitesimal transition (interpretation).}
For small $h>0$ and $i\neq j$,
\[
\Pr(X_{\mathrm{nm}}(t+h)=j \mid X_{\mathrm{nm}}(t)=i, x_0)
= K_{ij}(t)\,h + o(h)
= \big(R_{ij}(t) + \lambda(t)\mu^{\mathrm{abs}}_j(t)\big)h + o(h),
\]
which is the continuous-time analogue of ``either follow the base dynamics or refresh from the $x_0$-marginal''.




==> includes/mixed.tex <==
\begin{equation}
    p(\z_{t+1} \mid \z_t, x)
    \;=\;
    \Normal\!\big(\z_t + \alpha_t\,\e_x,\; \beta_t I\big).
\end{equation}
\begin{equation}
    p(\x_{t} \mid \x_s, x)
    \;=\;
    \Cat\!\big(\gamma_{t\mid s}\x_s + (1-\gamma_{t\mid s})\e_x \big),
\end{equation}
with $\gamma_{t\mid s}=\frac{\gamma_t}{\gamma_s}$.

Marginal:
\begin{equation}
    p(\z_t \mid \z_0, x)
    \;=\;
    \Normal\Big(\z_t + \sum_{i=0}^t\alpha_i\,\e_x,\; \sum_{i=0}^t\beta_i I\Big).
\end{equation}

\begin{equation}
p(\x_t \mid \x_0, x)
\;=\;
\Cat\!\Big(\gamma_{t}\,\x_0 \;+\; (1-\gamma_{t})\,\e_x\Big).
\end{equation}
\begin{equation}
p(\x_t \mid x)
\;=\;
\Cat\!\Big(\gamma_{t}\,q_0 \;+\; (1-\gamma_{t})\,\e_x\Big).
\end{equation}


\begin{equation}
    p(\x_s\mid\x_t,x)=\Cat(\frac{Q_{t\mid s}\x_t\cdot Q_s^T\e_x}{\x_tQ_t^T\e_x})
\end{equation}

% Let the time-s marginal be
\begin{align}
\pi_s \;:=\; p(\x_s\mid x) \;=\; \gamma_s q_0 + (1-\gamma_s)\e_x, \\
\pi_s(x) \;:=\; \e_x^\top \pi_s \;=\; (1-\gamma_s)+\gamma_s\,q_0(x).
\end{align}

Forward process:
\begin{equation}
p(\x_s\mid \x_t,x)
=
\begin{cases}
\Cat(\x_t), & \text{if }\x_t\neq \e_x,\\[6pt]
\Cat\!\Bigg(\displaystyle
\frac{(1-\gamma_{t\mid s})\,\pi_s \;+\; \gamma_{t\mid s}\,\pi_s(x)\,\e_x}
{(1-\gamma_{t\mid s}) \;+\; \gamma_{t\mid s}\,\pi_s(x)}
\Bigg), & \text{if }\x_t=\e_x.
\end{cases}
\end{equation}


\[
p(\x_s\mid \x_t=\e_x,x)
=
\Cat\!\Bigg(
\frac{(1-\gamma_{t\mid s})\big(\gamma_s q_0+(1-\gamma_s)\e_x\big)
\;+\;\gamma_{t\mid s}\big((1-\gamma_s)+\gamma_s q_0(x)\big)\e_x}
{(1-\gamma_{t\mid s})+\gamma_{t\mid s}\big((1-\gamma_s)+\gamma_s q_0(x)\big)}
\Bigg).
\]


Reverse process:

\begin{align}
p(\x_{t}\mid \x_{s},x)
&=\Cat\!\Big((1-\lambda)\big[\gamma_{t\mid s}\,\x_s+(1-\gamma_{t\mid s})\e_x\big]
+\lambda\big[\gamma_t q_0+(1-\gamma_t)\e_x\big]\Big)\\
&=\Cat\!\Big((1-\lambda)\gamma_{t\mid s}\,\x_s
+\lambda\gamma_t q_0
+\Big((1-\lambda)(1-\gamma_{t\mid s})+\lambda(1-\gamma_t)\Big)\e_x\Big)\\
&=\Cat\!\Big((1-\lambda)\gamma_{t\mid s}\,\x_s
+\lambda\gamma_t q_0
+\Big(1-\big((1-\lambda)\gamma_{t\mid s}+\lambda\gamma_t\big)\Big)\e_x\Big).
\end{align}

Define
\[
A_{t\mid s} := (1-\lambda)\gamma_{t\mid s} + \lambda \gamma_t,
\qquad
\tilde\gamma_{t\mid s} := 1-A_{t\mid s} = (1-\lambda)(1-\gamma_{t\mid s})+\lambda(1-\gamma_t).
\]
If \(A_t>0\), define the blended state
\[
\tilde q_{t\mid s} := \frac{(1-\lambda)\gamma_{t\mid s}\,\x_t + \lambda \gamma_t\,q_0}{A_t}.
\]
Then the transition can be written as
\[
p(\x_{t+1}\mid \x_t,x)
=
\Cat\!\Big((1-\tilde\gamma_{t\mid s})\,\tilde q_t + \tilde\gamma_{t\mid s}\,\e_x\Big).
\]
(If \(A_t=0\), then \(\tilde\gamma_t=1\) and the transition is simply \(\Cat(\e_x)\).)
\clearpage
ELBO:
$\lambda=0$:
\begin{align}
    \log p_\theta(x)
    &\geq
    \mathbb{E}_{p(\x_1, \dots,\x_k\mid x)}\left[
    \log \frac{p_\theta(x,\x_1, \dots,\x_k)}{p(\x_1, \dots,\x_k\mid x)}
    \right] \\
    &=
    \mathbb{E}_{p(\x_1,\dots,\x_k\mid x)}\!\left[\log p(x\mid \x_k)\right] \\
    \;&-\;
    \sum_{i=0}^{k-1}
    \mathbb{E}_{p(\x_i\mid x)}\!\left[
    \mathrm{KL}\!\left( p(\x_{i+1}\mid \x_i,x)\,\big\lVert\, p_\theta(\x_{i+1}\mid\x_i) \right)\right] \\
    &=
    \mathbb{E}_{p(\x_1,\dots,\x_k\mid x)}\!\left[\log p(x\mid \x_k)\right] \\
    \;&-\;
    \sum_{i=0}^{k-1}
    \mathbb{E}_{p(\x_{i+1},\x_i\mid x)}\!\left[
    - \log p_\theta(\x_{i+1}\mid\x_i) \right] + C \\
    &=
    \mathbb{E}_{p(\x_1,\dots,\x_k\mid x)}\!\left[\log p(x\mid \x_k)\right] \\
    \;&+\;
    \sum_{i=0}^{k-1}
    \mathbb{E}_{p(\x_i\mid x)}\!\left[
     (1-\gamma_{i+1\mid i})\log p_\theta(\e_x\mid\x_i) \right] + C. 
\end{align}
$1-\gamma_{i+1\mid i}=1-\frac{\gamma_{i+1}}{\gamma_i}=\frac{\gamma_{i}-\gamma_{i+1}}{\gamma_i}$

$\lambda\neq 0:$
\begin{align}
\log p_\theta(x)
\ge\;
&\mathbb{E}_{p(\x_{1:k}\mid x)}\!\big[\log p_\theta(x\mid \x_k)\big] \\
&+\sum_{i=0}^{k-1}\mathbb{E}_{p(\x_i\mid x)}\Big[
w_i^{\x_i}\log p_\theta(\x_i\mid \x_i)
+w_i^{x}\log p_\theta(\e_x\mid \x_i)
+w_i^{q_0}\,\mathbb{E}_{c\sim q_0}\log p_\theta(\e_c\mid \x_i)
\Big] \;+\; C,
\end{align}
\[
w_i^{\x_i}=(1-\lambda)\gamma_{i+1\mid i},\qquad
w_i^{q_0}=\lambda\gamma_{i+1},\qquad
w_i^{x}=(1-\lambda)(1-\gamma_{i+1\mid i})+\lambda(1-\gamma_{i+1}),
\]


\clearpage

% Bridge (consistent with the marginal below):
\begin{equation}
    p(\x_{t} \mid \x_s, x)
    \;=\;
    \Cat\!\Big(\gamma_{t\mid s}\,\x_s \;+\; (1-\gamma_{t\mid s})\,\e_x \Big),
\end{equation}
with \(\gamma_{t\mid s}=\frac{\gamma_t}{\gamma_s}\) (for \(t\ge s\)).

% Marginal (assume \gamma_0=1):
\begin{equation}
    p(\x_t \mid \x_0, x)
    \;=\;
    \Cat\!\Big(\gamma_{t}\,\x_0 \;+\; (1-\gamma_{t})\,\e_x\Big).
\end{equation}

% Mixture transition (no \bar\gamma):
\begin{align}
p(\x_{t}\mid \x_{s},x)
&=\Cat\!\Big((1-\lambda)\big[\gamma_{t\mid s}\,\x_s+(1-\gamma_{t\mid s})\e_x\big]
+\lambda\big[\gamma_t q_0+(1-\gamma_t)\e_x\big]\Big)\\
&=\Cat\!\Big((1-\lambda)\gamma_{t\mid s}\,\x_s
+\lambda\gamma_t q_0
+\Big((1-\lambda)(1-\gamma_{t\mid s})+\lambda(1-\gamma_t)\Big)\e_x\Big)\\
&=\Cat\!\Big((1-\lambda)\gamma_{t\mid s}\,\x_s
+\lambda\gamma_t q_0
+\Big(1-\big((1-\lambda)\gamma_{t\mid s}+\lambda\gamma_t\big)\Big)\e_x\Big).
\end{align}

\textcolor{red}{Double check wq0}\\
Define
\[
A_{t\mid s} := (1-\lambda)\gamma_{t\mid s} + \lambda \gamma_t,
\qquad
\tilde\gamma_{t\mid s} := 1-A_{t\mid s}.
\]
If \(A_{t\mid s}>0\), define the blended state
\[
\tilde q_{t\mid s} := \frac{(1-\lambda)\gamma_{t\mid s}\,\x_s + \lambda \gamma_t\,q_0}{A_{t\mid s}}.
\]
Then the transition can be written as
\[
p(\x_{t}\mid \x_s,x)
=
\Cat\!\Big(A_{t\mid s}\,\tilde q_{t\mid s} + (1-A_{t\mid s})\,\e_x\Big)
=
\Cat\!\Big((1-\tilde\gamma_{t\mid s})\,\tilde q_{t\mid s} + \tilde\gamma_{t\mid s}\,\e_x\Big).
\]
(If \(A_{t\mid s}=0\), then \(\tilde\gamma_{t\mid s}=1\) and the transition is simply \(\Cat(\e_x)\).)

\clearpage
\begin{align}
p(\x_{s}\mid \x_{t}, x)
&=\Cat\!\Big(
(1-\lambda)\big[\gamma_{s\mid t}\,\x_t+(1-\gamma_{s\mid t})\e_x\big]
+\lambda\big[(1-\gamma_s) q_1+ \gamma_s\e_x\big]
\Big)\\
&=\Cat\!\Big(
(1-\lambda)\gamma_{s\mid t}\,\x_t
+\lambda(1-\gamma_s)q_1
+\Big((1-\lambda)(1-\gamma_{s\mid t})+\lambda \gamma_s\Big)\e_x
\Big)\\
&=\Cat\!\Big(
(1-\lambda)\gamma_{s\mid t}\,\x_t
+\lambda(1-\gamma_s) q_1
+\Big(1-\big((1-\lambda)\gamma_{s\mid t}+\lambda(1-\gamma_s)\big)\Big)\e_x
\Big).
\end{align}

\[
A_{s\mid t} := (1-\lambda)\gamma_{s\mid t} + \lambda (1-\gamma_s),
\qquad
\tilde\gamma_{s\mid t} := 1-A_{s\mid t}.
\]

If \(A_{s\mid t}>0\), define the blended state
\[
\tilde q_{s\mid t} := \frac{(1-\lambda)\gamma_{s\mid t}\,\x_t + \lambda (1-\gamma_s)\,q_1}{A_{s\mid t}}.
\]

The transition can be written as
\[
p(\x_{s}\mid \x_t,x)
=
\Cat\!\Big(A_{s\mid t}\,\tilde q_{s\mid t} + (1-A_{s\mid t})\,\e_x\Big)
=
\Cat\!\Big((1-\tilde\gamma_{s\mid t})\,\tilde q_{s\mid t} + \tilde\gamma_{s\mid t}\,\e_x\Big).
\]

For $\lambda=0$:

\begin{align}
p(\x_{s}\mid \x_{t}, x)
&=\Cat\!\Big(
\gamma_{s\mid t}\,\x_t
+\big(1-\gamma_{s\mid t}\big)\e_x
\Big).
\end{align}


\clearpage
\paragraph{Notations:}
$\x_t$ is a discrete random variable taking values in $\{1,\dots,K\}$, represented in one-hot encoding.  $\Cat(\cdot)$ denotes a categorical distribution with the given probability vector. Let $x \sim D$ be a datapoint sampled from the data. We denote the corresponding one-hot vector by $\e_x \in \Delta^{K-1}$. We consider a prior distribution $q_1 \in \Delta^{K-1}$.

\paragraph{Discrete-time forward process}

The marginal distribution at time $t$ is defined as:
%\begin{align}
%p_{\lambda}(\x_t \mid x)
%&=
%\Cat\!\Big(
%\x_t;\,
%\big(1-((1-\lambda)\alpha_t+\lambda\gamma_t\big))\,q_0\\
%&\qquad+ 
%\Big(\big((1-\lambda)\alpha_t+\lambda\gamma_t\big)\Big)\,\mathbf \e_x
%\Big),
%\end{align}
%where $\alpha_{t} \in [0,1]$ and $\gamma_t = 1 - \alpha_t$.

%For $\lambda = 0$:

\begin{align}\label{eq:marignal}
p_{0}(\x_t \mid x) &= \Cat\!\Big(
\x_t;\, (1-\alpha_t) q_1 + \alpha_t \e_x \Big)\\
&= \Cat\!\Big(
\x_t;\, \gamma_t q_1 + (1-\gamma_t) \e_x \Big),
\end{align}
where $\gamma_t \in [0,1]$ is a noise scheduler, and $\alpha_t = 1-\gamma_t$.

%For $\lambda = 1$: 
%\begin{equation}
%p_{1}(\x_t \mid x) = \Cat\!\Big(
%\x_t;\, (1-\gamma_t) q_0 + \gamma_t \e_x \Big)
%\end{equation}


\paragraph{Discrete-time reverse process}

\begin{align}
p_{\lambda}(\x_{s}\mid \x_{t},x)
&=\Cat\!\Big(\x_s; (1-\lambda)\big[\gamma_{s\mid t}\,\x_t+(1-\gamma_{s\mid t})\e_x\big] \\
&\qquad
+\lambda\big[\gamma_s q_1+(1-\gamma_s)\e_x\big]\Big),
\end{align}
where $\lambda \in [0,1]$.

\subsection{For $\lambda = 0$:}

\paragraph{Discrete-time forward process} is non-Markovian and is defined as:

%\begin{equation}
%p_0(\x_t \mid \x_s, x)
%=
%\begin{cases}
%\Cat(\x_t; \x_s),
%& \x_s \neq x, \\[6pt]
%\Cat(\x_t; \dfrac{\alpha_t}{\alpha_s}\,\ \e_x
%+
%\Big(1-\dfrac{\alpha_t}{\alpha_s}\Big) q_0,
%& \x_s = x
%\end{cases}
%\end{equation}
\begin{equation}
p_0(\x_t\mid \x_s,x)
=
\begin{cases}
\Cat(\x_t; \x_s), &\x_s\neq \e_x,\\
\Cat\!\Bigg(\displaystyle
\frac{(1-\gamma_{s\mid t})\,\pi_t \;+\; \gamma_{s\mid t}\,\pi_t(x)\,\e_x}
{(1-\gamma_{s\mid t}) \;+\; \gamma_{s\mid t}\,\pi_t(x)}
\Bigg), & \x_s=\e_x,
\end{cases}
\end{equation}

where 
% Let the time-s marginal be
\begin{align}
\pi_t \;:=\; p(\x_t\mid x) \;=\; \gamma_t q_1 + (1-\gamma_t)\e_x, \\
\pi_t(x) \;:=\; \e_x^\top \pi_t \;=\; (1-\gamma_t)+\gamma_t\,q_1(x).
\end{align}

The induced marginal distribution $p(\x_t | x)$ corresponds to \cref{eq:marignal}.

\begin{itemize}
    \item TODO: provide proof
\end{itemize}

%\textit{Proof.} Proof by induction. 
%We start with $p(\x_{t_1} \mid x) =
%\Cat\!\Big(\x_{t_1}; (1-\alpha_{t_1})\,q_0 \;+\; \alpha_{t_1}\,\e_x\Big).$ 
%Assume that $p(\x_t \mid x) =
%\Cat\!\Big(\x_t; (1-\alpha_{t})\,q_0 \;+\; \alpha_{t}\,\e_x\Big).$
%We want to check if $p(\x_s \mid x) =
%\Cat\!\Big(\x_s; (1-\alpha_{s})\,q_0 \;+\; \alpha_{s}\,\e_x\Big),$ for $s < t$.

%\begin{align}
%p(\mathbf x_s=\mathbf e_x \mid x)
%&= \sum_{\mathbf x_t} p(\mathbf x_s=\mathbf e_x \mid \mathbf x_t, x)\,p(\mathbf x_t\mid x) \\
%&= p(\mathbf x_s=\mathbf e_x \mid \mathbf x_t=\mathbf e_x, x)\,p(\mathbf x_t=\mathbf e_x\mid x)\\
%&\quad \;+\;
%\sum_{\mathbf x_t\neq \mathbf e_x} p(\mathbf x_s=\mathbf e_x \mid \mathbf x_t, x)\,p(\mathbf x_t\mid x).
%\end{align}

%\begin{align}
%p(\mathbf x_s=\mathbf e_x \mid x)
%&= \frac{\alpha_s}{\alpha_t} \times \alpha_t + 0   = \alpha_s
%\end{align}
%Similarly, for $\mathbf x_s\neq \mathbf e_x$ we have
%\begin{align}
%p(\mathbf x_s\neq \mathbf e_x \mid x)
%&=1-p(\mathbf x_s=\mathbf e_x\mid x)
%=1 - \alpha_s,
%\end{align}
%which matches the claimed marginal.




\paragraph{Discrete-time reverse process:}

This corresponds to an absorbing diffusion process towards the data token.
\begin{equation}\label{eq:posterior_0}
p_0(\x_{s}\mid \x_{t},x)
=\Cat\!\big(\x_s; \gamma_{s\mid t}\,\x_t+(1-\gamma_{s\mid t})\e_x\big),
\end{equation} 
where $\gamma_{s\mid t} = \frac{1-\alpha_s}{1-\alpha_t} = \frac{\gamma_s}{\gamma_t}.$

Check for $\x_t = e_x$:
\begin{equation}
p_0(\x_{s}\mid \x_{t} = \e_x,x)
=\Cat\!\big(\x_s; \e_x\big)
\end{equation}
$\e_x$ is absorbing.

Check for $\x_t = e_y, y \neq x$:
\begin{equation}
p_0(\x_{s}\mid \x_{t} = \e_y,x)
=\Cat\!\big(\gamma_{s\mid t}\,\e_y+(1-\gamma_{s\mid t})\e_x\big)
\end{equation}
every other state $\x_t \neq \e_x$ is non-absorbing.

Reordering the states so that \(x\) is last, the corresponding transition matrix is
\[
P^{0}_{s\mid t}
=
\begin{pmatrix}
\gamma_{s\mid t} & 0 & \cdots & 0 & 1-\gamma_{s\mid t} \\
0 & \gamma_{s\mid t} & \cdots & 0 & 1-\gamma_{s\mid t} \\
\vdots & & \ddots & & \vdots \\
0 & 0 & \cdots & \gamma_{s\mid t} & 1-\gamma_{s\mid t} \\
0 & 0 & \cdots & 0 & 1
\end{pmatrix}.
\]

\paragraph{Parametrized transition matrix.}
 the parametrized transition matrix
$P^{\theta}_{s\mid t}\in\mathbb{R}^{K\times K}$ is given by
\[
P^{\theta}_{s\mid t}
=
\begin{pmatrix}
\gamma + (1-\gamma)\mu_{11} & (1-\gamma)\mu_{12} & \cdots &  (1-\gamma)\mu_{1K} \\
(1-\gamma)\mu_{21} & \gamma + (1-\gamma)\mu_{22} & \cdots & (1-\gamma)\mu_{2K} \\
\vdots & & \ddots &  \vdots \\
(1-\gamma)\mu_{K-1,1} & (1-\gamma)\mu_{K-1,2} & \cdots & (1-\gamma)\mu_{K-1,K} \\
(1-\gamma)\mu_{K1} & (1-\gamma)\mu_{K2} & \cdots & \gamma + (1-\gamma)\mu_{KK}
\end{pmatrix},
\]
where
\[
\mu_{jk} := \mu_{\theta,k}\!\left(x_t = e_j,\, s\right),
\]
and 
\[
\mu_\theta(x_t,t)\in\Delta^{K-1}
\]
is the probability vector output by the network.

TBD:
\begin{itemize}
    \item Double-check the corresponding ELBO
    \item Formalize how this is different from standard MDM
    \item Formalize how this is different from uniform DM
\end{itemize}

\subsubsection{ELBO for $\lambda = 0$:}
\begin{align}
&\log p(x) \geq \\ 
&\mathbb{E}_{p(x_{t_1} \mid x)}[\log p(x | x_{t_1})] - \mathrm{KL}\!\left( p(\x_1 \mid x) \,\big\lVert\, 
q_1(\x_1)\right)- L_T,
\end{align}

where:
\begin{align}
    L_T &= \sum_{i=1}^{k}
    \mathbb{E}_{p(\x_i\mid x)}\!\left[
    \mathrm{KL}\!\left( p(\x_{i-1}\mid \x_i,x)\,\big\lVert\, p_\theta(\x_{i-1}\mid\x_i) \right)\right]\\
\end{align}

\paragraph{Case 1: the absorbing case where $\x_i = \e_x$}
\begin{align}
&\mathrm{KL}\!\left( p(\x_{i-1}\mid \x_i = \e_x,x)\,\big\lVert\, p(\x_{i-1}\mid \x_i = \e_x, \mu_{\theta}(\x_i, i)) \right)\\
&= p(\x_{i-1} = \e_x \mid \x_i = \e_x,x) \times\ \\
&\qquad\log \frac{p(\x_{i-1} = \e_x \mid \x_i = \e_x,x)}{p(\x_{i-1} = \e_x\mid \x_i = \e_x, \mu_{\theta}(\x_i, i))} \;+\; \\
&\qquad \sum_{j \neq x} p(\x_{i-1} = j \mid \x_i = \e_x,x) \times \\
&\qquad \log \frac{p(\x_{i-1} = j \mid \x_i = \e_x,x)}{p(\x_{i-1} = j \mid \x_i = \e_x, \mu_{\theta}(\x_i, i))}\\
&= 1 \times \log \frac{1}{p(\x_{i+1} = \e_x \mid \x_i = \e_x, \mu_{\theta}(\x_i, i))} \;+\; 0\\
&= - \log (\gamma_{i+1|i} +  (1 - \gamma_{i+1|i}) \e_x^{T} \mu_{\theta}(\x_i, i))
\end{align}
If the network perfectly recovers $\e_x$, then $\e_x^{T}\mu_{\theta}(\x_i,i) = 1$ and the loss equals 0.  Following the posterior in \cref{eq:posterior_0}, $p(\x_{i-1} = j \mid \x_i = \e_x,x) = 0 \text{ for } j \neq \e_x$, and we use the $x_0$-parametrization $p_{\theta}(\x_{i-1} \mid \x_i) = \Cat\big(\x_{i-1}; \gamma_{i-1|i}\x_i + (1 - \gamma_{i-1|i}) \mu_{\theta}(\x_i, i)\big)$.


\paragraph{Case 2: The non-absorbing case where $\x_i = \e_y, \e_y \neq \e_x$}
Here, the true posterior has support over $\{\e_y, \e_x\}$

\begin{align}
&\mathrm{KL}\!\left( p(\x_{i-1}\mid \x_i = \e_y,x)\,\big\lVert\, p(\x_{i-1}\mid \x_i = \e_y, \mu_{\theta}(\x_i, i)) \right)\\
&= \gamma_{i-1|i} \log \frac{\gamma_{i-1|i}}{\gamma_{i-1|i} + (1-\gamma_{i-1|i})\mu_{\theta,y}(\e_y, i))} \;+\; \\
&\qquad (1-\gamma_{i-1|i}) \log \frac{(1-\gamma_{i-1|i})}{(1-\gamma_{i-1|i}) \mu_{\theta,x}(\e_y, i)}\\
&= \gamma_{i-1|i} \log \frac{\gamma_{i-1|i}}{\gamma_{i-1|i}+ (1-\gamma_{i-1|i}) \e_y^{T}\mu_{\theta}(\e_y, i)} \;-\; \\
&\qquad (1-\gamma_{i-1|i}) \log \e_x^{T}\mu_{\theta}(\e_y, i)
\end{align}

\paragraph{Unified Expression.}
Using indicator notation $\mathbf{1}[\cdot]$, both cases can be written as
\[
\begin{aligned}
&\mathrm{KL}\!\left(
p_0(\cdot \mid \x_i)
\;\middle\|\;
p_\theta(\cdot \mid \x_i)
\right)\\
&\quad =
\mathbf{1}[\x_i = \e_x]\,
\Big(
-\log\!\big(
\gamma + (1-\gamma)\, \e_x^\top \mu_\theta(\x_i,i)
\big)
\Big)
\\
&\quad
+
\mathbf{1}[\x_i \neq \e_x]\,
\Bigg[
\gamma \log\!\Bigg(
\frac{\gamma}{
\gamma + (1-\gamma)\, \x_i^\top \mu_\theta(\x_i,i)}
\Bigg)
+
(1-\gamma)\log\!\Bigg(
\frac{1}{
\e_x^\top \mu_\theta(\x_i,i)}
\Bigg)
\Bigg].
\end{aligned}
\]


\subsection{For $\lambda = 1$}

For $\lambda = 1$, the reverse process completely ignores $\x_t$. We resample $\x_s$ from a fixed mixture of prior distribution $q_1$ with probability $\gamma_s$, and the clean token $x$ with probability $1-\gamma_s$. The posterior is defined as:
\begin{align}
p_1(\x_{s}\mid \x_{t},x) = p(\x_s \mid x) 
&=\Cat\!\big(\x_s; \gamma_s q_1+ (1-\gamma_s)\e_x\big).
\end{align}
 
The forward process is non-Markovian as the latents $\x_s$ and $\x_t$ are conditionally independent given $x$:
\begin{equation}
    p_1(\x_t \mid \x_s, x) = p(\x_t | s) = \Cat\!\big(\x_t; \gamma_t q_1+ (1-\gamma_t) \e_x\big)
\end{equation}

TBD:
\begin{itemize}
    \item Compare to SID paper
    \item Double-check ELBO
\end{itemize}
\newpage










==> includes/non_markovian_discrete.tex <==
% Non-Markovian forward process built on top of the absorbing-[MASK] kernel

% State space: K real tokens plus an absorbing mask state m = [MASK]
\newcommand{\X}{\mathcal{X}}
\newcommand{\mask}{m}

Let $\X := \{1,\dots,K\}\cup\{\mask\}$, where \mask denotes the absorbing \texttt{[MASK]} token.
Let $\{\beta_t\}_{t=1}^T \subset [0,1]$ be the (masking) noise schedule and define
\[
\bar\alpha_t := \prod_{s=1}^t (1-\beta_s), \qquad \bar\alpha_0 := 1.
\]

% 1) Base (Markov) absorbing forward kernel q_abs(x_t | x_{t-1})
Define the (time-inhomogeneous) absorbing-mask forward kernel \(q_{\mathrm{abs}}\) by
\begin{align}
q_{\mathrm{abs}}(x_t \mid x_{t-1})
&=
\begin{cases}
1-\beta_t, & x_{t-1}=i\in\{1,\dots,K\},\; x_t=i,\\
\beta_t,   & x_{t-1}=i\in\{1,\dots,K\},\; x_t=\mask,\\
1,         & x_{t-1}=\mask,\; x_t=\mask,\\
0,         & \text{otherwise.}
\end{cases}
\end{align}

% 2) Closed-form t-step marginal from x0 under the absorbing kernel
Its \(t\)-step marginal from \(x_0\) is
\begin{align}
q_{\mathrm{abs}}(x_t \mid x_0)
&=
\begin{cases}
\bar\alpha_t,        & x_0=i\in\{1,\dots,K\},\; x_t=i,\\
1-\bar\alpha_t,      & x_0=i\in\{1,\dots,K\},\; x_t=\mask,\\
1,                   & x_0=\mask,\; x_t=\mask,\\
0,                   & \text{otherwise.}
\end{cases}
\end{align}

% 3) Non-Markovian forward: occasional "refresh" from x0 (enables re-masking even if currently unmasked)
Introduce a latent switch \(s_t \sim \mathrm{Bernoulli}(\lambda_t)\), with \(\lambda_t\in[0,1]\), and define
\begin{align}
q_{\mathrm{nm}}(x_t \mid x_{t-1}, x_0, s_t)
&=
\begin{cases}
q_{\mathrm{abs}}(x_t \mid x_{t-1}), & s_t=0,\\
q_{\mathrm{abs}}(x_t \mid x_0),     & s_t=1.
\end{cases}
\end{align}
Marginalizing \(s_t\) gives the explicit non-Markov forward transition (non-Markov in \(x\) alone, but Markov in \((x,s)\)):
\begin{align}
q_{\mathrm{nm}}(x_t \mid x_{t-1}, x_0)
&=
(1-\lambda_t)\,q_{\mathrm{abs}}(x_t \mid x_{t-1})
\;+\;
\lambda_t\,q_{\mathrm{abs}}(x_t \mid x_0).
\end{align}

% (Optional) The resulting posterior over x_{t-1} is an exact mixture:
\begin{align}
q_{\mathrm{nm}}(x_{t-1} \mid x_t, x_0)
&=
(1-\lambda_t)\,q_{\mathrm{abs}}(x_{t-1} \mid x_t, x_0)
\;+\;
\lambda_t\,q_{\mathrm{abs}}(x_{t-1} \mid x_0),
\end{align}
where \(q_{\mathrm{abs}}(x_{t-1}\mid x_0)\) is the \((t\!-\!1)\)-step marginal (same closed form with \(\bar\alpha_{t-1}\)).


% Requires: \usepackage{amsmath,amssymb}
% Notation: absorbing forward kernel q_abs, and a non-Markov forward q_nm with "refresh" prob \lambda_t.

\newcommand{\MASK}{\mathtt{[MASK]}}

\paragraph{Non-Markov forward (refresh-from-$x_0$).}
Assume the forward transition is
\begin{equation}
q_{\mathrm{nm}}(x_t \mid x_{t-1}, x_0)
=
(1-\lambda_t)\,q_{\mathrm{abs}}(x_t \mid x_{t-1})
\;+\;
\lambda_t\,q_{\mathrm{abs}}(x_t \mid x_0),
\qquad \lambda_t\in[0,1].
\label{eq:qnm-forward}
\end{equation}

\paragraph{Claim (marginal is unchanged).}
For all $t\ge 0$,
\begin{equation}
q_{\mathrm{nm}}(x_t \mid x_0) \;=\; q_{\mathrm{abs}}(x_t \mid x_0).
\label{eq:marginal-unchanged}
\end{equation}

\paragraph{Proof (by induction).}
Base case $t=0$ is trivial: $q_{\mathrm{nm}}(x_0\mid x_0)=1=q_{\mathrm{abs}}(x_0\mid x_0)$.

Induction step: assume $q_{\mathrm{nm}}(x_{t-1}\mid x_0)=q_{\mathrm{abs}}(x_{t-1}\mid x_0)$. Then
\begin{align}
q_{\mathrm{nm}}(x_t \mid x_0)
&= \sum_{x_{t-1}} q_{\mathrm{nm}}(x_t \mid x_{t-1}, x_0)\; q_{\mathrm{nm}}(x_{t-1}\mid x_0) \\
&= \sum_{x_{t-1}} \Big[(1-\lambda_t)q_{\mathrm{abs}}(x_t\mid x_{t-1}) + \lambda_t q_{\mathrm{abs}}(x_t\mid x_0)\Big]\; q_{\mathrm{abs}}(x_{t-1}\mid x_0) \\
&= (1-\lambda_t)\sum_{x_{t-1}} q_{\mathrm{abs}}(x_t\mid x_{t-1}) q_{\mathrm{abs}}(x_{t-1}\mid x_0)
\;+\; \lambda_t q_{\mathrm{abs}}(x_t\mid x_0)\sum_{x_{t-1}} q_{\mathrm{abs}}(x_{t-1}\mid x_0) \\
&= (1-\lambda_t) q_{\mathrm{abs}}(x_t\mid x_0) \;+\; \lambda_t q_{\mathrm{abs}}(x_t\mid x_0) \\
&= q_{\mathrm{abs}}(x_t\mid x_0),
\end{align}
where we used (i) Markov composition of $q_{\mathrm{abs}}$ for the first sum, and (ii) normalization
$\sum_{x_{t-1}} q_{\mathrm{abs}}(x_{t-1}\mid x_0)=1$ for the second sum. This proves \eqref{eq:marginal-unchanged}.

\paragraph{Closed form for absorbing-mask.}
Define $\bar\alpha_t := \prod_{s=1}^t (1-\beta_s)$, $\bar\alpha_0:=1$. Then, for $x_0=i\in\{1,\dots,K\}$,
\begin{equation}
q_{\mathrm{nm}}(x_t=i \mid x_0=i)=\bar\alpha_t,\qquad
q_{\mathrm{nm}}(x_t=\MASK \mid x_0=i)=1-\bar\alpha_t,\qquad
q_{\mathrm{nm}}(x_t=j \mid x_0=i)=0\ (j\neq i),
\end{equation}
and if $x_0=\MASK$, then $q_{\mathrm{nm}}(x_t=\MASK\mid x_0=\MASK)=1$.



==> tables/app_lm1b_samples.tex <==
\begin{table}[t]
\centering
\caption{Generated samples for unconditional generation from IDMM trained on LM1B.}
\label{tab:idmm_samples}
\begin{tabular}{c p{0.78\linewidth}}
\toprule
\textbf{T} & \textbf{Generated Text} \\
\midrule
256 &

\\ \hline
&

\\ \hline
&

\\
\midrule
512 &
\\ \hline
&
\\ \hline
&
 \\
\midrule
1024 &
\\ \hline
&
 \\ \hline
&
\\
\bottomrule
\end{tabular}
\end{table}

